The Manifold Density Function: An Intrinsic Method for the Validation of Manifold Learning

We introduce the manifold density function, which is an intrinsic method to validate manifold learning techniques. Our approach adapts and extends Ripley's $K$-function, and categorizes in an unsupervised setting the extent to which an output of a manifold learning algorithm captures the structure of a latent manifold. Our manifold density function generalizes to broad classes of Riemannian manifolds. In particular, we extend the manifold density function to general two-manifolds using the Gauss-Bonnet theorem, and demonstrate that the manifold density function for hypersurfaces is well approximated using the first Laplacian eigenvalue. We prove desirable convergence and robustness properties.

==> body/append/exp.tex <==
% In the following section we outline additional experimental details left out for
% brevity in the main body of the paper.
% Our anonymized code is accessible at the following url for reproducibility:
% \href{https://anonymous.4open.science/r/intrinsic-manifold-validation/README.md}{https://anonymous.4open.science/r/intrinsic-manifold-validation/}

% \subsection{Additional Experimental Details for Surfaces}

% In the main paper, we presented results for surfaces
% delineating between uniform samples and stratifications.
% Here, we present more explicitly the details regarding how these samples were generated,
% alongside additional anicdotal experimental results not included in the main body.

% We begin with a discussion of the manifold score on the Klein bottle, and implement
% the comparison of manifold learning algorithms shown in \figref{klein} in \secref{prelim}.
% This anecdote provides a sense for both the intended positive behavior and the shortcomings
% of our use of the \ourkf, which appear inherent to intrinsic validation in general.
% Namely, we lift a parameterization of the Klein bottle in $\R^3$ to ten dimensions by
% assigning values from the interval $[0,2\pi]$ uniformly at random to each of the other
% seven coordinates. In total, this point cloud representation lying on an ambient Klein
% bottle in 3D has 1000 points. 
% We then attempt to re-learn the 3D parameterization of the
% Klein bottle; computing embeddings in $\R^3$ of the point cloud in $\R^10$ using PCA, ISOMAP,
% t-SNE, LLE, and spectral embedding, each with $n_components=3$ and $n_neighbors=6$.
% To the naked eye, PCA appears to perform the best, simply by dropping the
% other seven dimensions, and ISOMAP also appears to perform well, albeit a bit worse. In actuality,
% ISOMAP assigns much greater density to the handle region of the Klein bottle in this example,
% and achieves a somewhat unfavorable score. This provides an adversarial example where t-SNE outperforms ISOMAP, despite the visual
% preferability of the latter.
% The results when evaluating the manifold score on each algorithm are summarized in the following table,
% where we report the manifold score on the \ourkf restricted to radius $r=0.3$:

% \begin{table}[H]
%     \caption{Differing Manifold Scores from the Klein Bottle}
%     \begin{center}
%     \begin{tabular}{lllll}
%     \textbf{PCA}  &\textbf{ISOMAP} & \textbf{t-SNE} & \textbf{LLE} & \textbf{Spectral Embedding} \\
%     \hline \\
%     $0.9557$ & $0.7179$ & $0.9154$ & $0.3988$ & $0.6881$
%     \end{tabular}
%     \end{center}
% \end{table}

% \begin{figure}[htbp]
%     \floatconts
%     {fig:klein_embeddings_bad}% label for whole figure
%     {\caption{Embeddings of the Klein bottle in $\mathbb{R}^3$ projected from $\mathbb{R}^{10}$.}}% caption for whole figure
%     {%
%         \subfigure{%
%         \label{fig:pca_klein_bad}% label for this sub-figure
%         \includegraphics[width=0.31\textwidth]{figs/klein_pca_bad}
%         }\qquad % space out the images a bit
%         \subfigure{%
%         \label{fig:iso_klein_bad}% label for this sub-figure
%         \includegraphics[width=0.31\textwidth]{figs/klein_iso_bad}
%         }\qquad % space out the images a bit
%         \subfigure{%
%         \label{fig:tsne_klein_bad}% label for this sub-figure
%         \includegraphics[width=0.31\textwidth]{figs/klein_tsne_bad}
%         }\\ % break line to the next row of subfigures
%         \subfigure{%
%         \label{fig:lle_klein_bad}% label for this sub-figure
%         \includegraphics[width=0.31\textwidth]{figs/klein_lle_bad}
%         }\qquad % space out the images a bit
%         \subfigure{%
%         \label{fig:spectral_klein_good}% label for this sub-figure
%         \includegraphics[width=0.31\textwidth]{figs/klein_spec}
%         }
%     }
% \end{figure}


% \begin{figure}[H]
%     \centering
%     \includegraphics[width=0.9\textwidth]{figs/klein_kfcn}
% \end{figure}


% Upon visual inspection, the apparent best performing algorithm in this example (PCA) is indeed detected as performing well,
% while the worse performing algorithms are generally detected as such. However, the manifold score is not able to distinguish between
% ISOMAP and t-SNE in the example, despite visually ISOMAP appearing to better uncover the manifold.
% This illuminates a shortcoming of the manifold score; which is a consequence of working in the unsupervised setting.
% That is, without knowledge of the ground truth manifold which we are attempting to uncover,
% there is no way of distinguishing between a uniform sample of something more distantly resembling a desired manifold,
% and a nonuniform sample closely resembling a desired manifold.



% \subsection{Experimental Details for Hypersurfaces}

% In what follows, we outline the resulting \ourkfs for hyperspheres,
% tabulated in their corresponding dimension. We provide a more complete experiment here,
% including edge cases in lower and higher dimensions than the cases included in experiments
% in the main body. Interestingly, only upon reaching five dimensions does scaling
% the \ourkf for hypersurfaces become beneficial, which we attribute to the fact that
% our scaling is indeed approximate; if possible to work with two-manifolds the exact scaling
% afforded by the Gauss-Bonnet theorem is preferable.
% In very high dimensions, as expected, it becomes increasingly subtle (but still possible
% outside of the range of error)
% to distinguish between uniform samples nonuniform samples such as the stratification. Once again,
% we employ a stratification of two $d/2$ hyperspheres sampled on the surface of the $d$-dimensional
% hypersphere.

% \begin{table}[h]
%     \caption{Results on Hyperspheres of Differing Dimension} \label{exp:klein}
%     \begin{center}
%     \begin{tabular}{llll}
%     \textbf{Dimension}  &\textbf{Post Scaling} & \textbf{Pre Scaling} & \textbf{Stratification} \\
%     \hline \\
%     3             & $0.6801 \pm 0.0074$ & $0.7791 \pm 0.0093$ & $0.6251 \pm 0.0016$ \\
%     4             & $0.9143 \pm 0.0043$ & $0.9785 \pm 0.0046$ & $0.8291 \pm 0.0899$ \\
%     5             & $0.9823 \pm 0.0006$ & $0.9207 \pm 0.0049$ & $0.7936 \pm 0.0805$ \\
%     20             & $0.9983 \pm 0.00002$ & $0.9732 \pm 0.0003$ & $0.9842 \pm 0.0015$ \\
%     50             & $0.9997 \pm 0.000001$ & $0.9736 \pm 0.00012$ & $0.9982 \pm 0.000039$ \\
%     100             & $0.9999 \pm 0.0000003$ & $0.9735 \pm 0.00013$ & $0.9995 \pm 0.0000085$ \\
%     \end{tabular}
%     \end{center}
%   \end{table}

